Multi-label Classification with Partial Annotations using Class-aware Selective Loss

Large-scale multi-label classification datasets are commonly, and perhaps inevitably, partially annotated. That is, only a small subset of labels are annotated per sample. Different methods for handling the missing labels induce different properties on the model and impact its accuracy. In this work, we analyze the partial labeling problem, then propose a solution based on two key ideas. First, un-annotated labels should be treated selectively according to two probability quantities: the class distribution in the overall dataset and the specific label likelihood for a given data sample. We propose to estimate the class distribution using a dedicated temporary model, and we show its improved efficiency over a naive estimation computed using the dataset's partial annotations. Second, during the training of the target model, we emphasize the contribution of annotated labels over originally un-annotated labels by using a dedicated asymmetric loss. With our novel approach, we achieve state-of-the-art results on OpenImages dataset (e.g. reaching 87.3 mAP on V6). In addition, experiments conducted on LVIS and simulated-COCO demonstrate the effectiveness of our approach. Code is available at https://github.com/Alibaba-MIIL/PartialLabelingCSL.

==> draft-notes.tex <==
\label{draft-notes}

\textcolor{red}{
\textbf{Introduction:}
\begin{enumerate}
    \item Mention that the partial labeled is highly related to semi-supervised learning. We believe that our procedure may be valuable in the standard setting of semi-supervised learning. According to the paper "Realistic ... SSL", one of the challenges is the class-distribution: "Performance of SSL techniques can degrade drastically when the unlabeled data contains a different distribution of classes than the labeled data.". Hence, our solution may be related also in SSL and may be valuable there. Refernce: "Realistic Evaluation of Deep Semi-Supervised Learning Algorithms" (2019)
    \item Mention that we will present results using the MS-COCO dataset as it is fully-annotated and thus we can quantify true class frequencies and also, its annotation can be controlled 
\end{enumerate}
}

\textcolor{blue}{
\textbf{Section 2:}
\begin{enumerate}
    \item Define the multi-label loss with partial labels.
    \item Defining the two modes, and discuss their pros and cons
    \item Negative mode is better for ranking dominant labels, Ignore mode better preserves the class-distribution.
    \item Mention the challenge of frequent classes with Negative mode
    \item State that there is no one suit approach. Depends in annotation scheme, depends in class.
    \item Simulation details here or in the experimental study?
\end{enumerate}
}

